MapPrior: Bird's-Eye View Map Layout Estimation with Generative Models

Despite tremendous advancements in bird's-eye view (BEV) perception, existing models fall short in generating realistic and coherent semantic map layouts, and they fail to account for uncertainties arising from partial sensor information (such as occlusion or limited coverage). In this work, we introduce MapPrior, a novel BEV perception framework that combines a traditional discriminative BEV perception model with a learned generative model for semantic map layouts. Our MapPrior delivers predictions with better accuracy, realism, and uncertainty awareness. We evaluate our model on the large-scale nuScenes benchmark. At the time of submission, MapPrior outperforms the strongest competing method, with significantly improved MMD and ECE scores in camera- and LiDAR-based BEV perception.

==> supp_sec/abstract.tex <==
\begin{abstract}


In the supplementary material, we provide more qualitative results of BEV map segmentation and uncertainty quantification, as well as additional analysis on failure cases in Sec.~\ref{sec:qual}. 
In addition, we provide model architecture details in Sec.~\ref{sec:arch}. The video "MapPrior.mp4" briefly introduces our task, proposed solution, and compares our results with baseline models.
\end{abstract}


==> supp_sec/architectures.tex <==
\section{Model Architecture Details}


\label{sec:arch}
\paragraph{Predictive Stage} In the predictive stage, we are using BEVFusion\cite{bev_fusion}, with an unchanged model architecture. 
BEVFusion uses Swin-T\cite{liu2021swin} as the image backbone. It then applies FPN to fuse multi-scale camera features to produce a feature map of 1/8 input size. It downsamples camera images to 256×704. For the LiDAR backbone, BEVFusion adopts VoxelNet, using a voxel size of 0.1m. As a final step, BEVFusion uses a convolutional segmentation head to predict the BEV map.

\subsection{Auto-encoder}
We modified the model architecture from VQGAN\cite{VQGAN}. To make sure our input and output resolution of the BEV map is $200 \times 200$, and the latent space resolution is $12 \times 12$, we adjust the padding strategy in the auto-encoder model.

\paragraph{Encoder}
The encoder contains an input convolution layer followed by five downsampling blocks. Each downsampling block contains two res-net blocks. After downsampling, the encoder has two middle res-net blocks, one middle attention block, and one output convolution layer. We show detailed model architecture in Tab.~\ref{tab:Encoder}

\begin{table*}[!t]
\caption{Architecture for Encoder}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{layers} & \multicolumn{5}{|c|}{parameters} \\
\hline
input & Conv2d & \multicolumn{5}{|c|}{in\_ch:6, out\_ch: 128, kernel: 3x3, stride: 1, pad: 1 } \\
 \hline

\multirow{3}*{downsample\_block\_1} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128 } \\
~ &  Downsample(Conv2d) & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128,kernel:3x3, stride:2, padding=((0,1,0,1),val=0) } \\
\hline
\multirow{3}*{downsample\_block\_2} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128 } \\
~ &  Downsample(Conv2d) & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128,kernel:3x3, stride:2, padding=((0,1,0,1),val=0) } \\
\hline
\multirow{3}*{downsample\_block\_3} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 256 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256 } \\
~ &  Downsample(Conv2d) & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256,kernel:3x3, stride:2, padding=((0,1,0,1),val=0) } \\
\hline
\multirow{3}*{downsample\_block\_4} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256 } \\
~ &  Downsample(Conv2d) & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256,kernel:3x3, stride:2, padding=((0,1,0,1),val=0) } \\
\hline
\multirow{2}*{downsample\_block\_5} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 512 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256 } \\

\hline
\multirow{3}*{middle} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:512, out\_ch: 512 } \\
~ &  AttnBlock & \multicolumn{5}{|c|}{in\_ch:512 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:512, out\_ch: 512 } \\
\hline
\multirow{3}*{end} &  Normalize & \multicolumn{5}{|c|}{GroupNorm,num\_groups=32, num\_channels=512} \\

~ &  Activation & \multicolumn{5}{|c|}{x*sigmoid(x)} \\

~ &  Conv2d & \multicolumn{5}{|c|}{in\_ch:512, out\_ch: 256, kernel: 3x3, stride: 1, pad: 1 } \\
\hline
\end{tabular}
\label{tab:Encoder}
\end{table*}


\paragraph{Codebook}
The codebook has 1024 different tokens, each of which is a 256-dimensional feature vector. Empirically we find this size trade-offs well between the generator's capacity and inference speed. 

\paragraph{Decoder}
The decoder has a similar structure as the encoder. It contains an input convolution layer, two res-net blocks, and one attention layer before the upsampling blocks. It then includes five upsampling blocks, each containing three res-net blocks. Finally, the decoder applies an output convolution layer. We show the detailed model architecture in Tab.~\ref{tab:decoder}

\begin{table*}[!t]
\caption{Architecture for Decoder}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{layers} & \multicolumn{5}{|c|}{parameters} \\
\hline
\multirow{1}*{input} & Conv2d & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 512, kernel: 3x3, stride: 1, pad: 1 } \\

\hline
\multirow{3}*{middle} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:512, out\_ch: 512 } \\
~ &  AttnBlock & \multicolumn{5}{|c|}{in\_ch:512 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:512, out\_ch: 512 } \\
\hline


\multirow{3}*{upsample\_block\_1} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:512, out\_ch: 256 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256 } \\
\hline
\multirow{5}*{upsample\_block\_2} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256 } \\
~ &  Upsample(nearest\_interpolate) & \multicolumn{5}{|c|}{scale\_factor=2.0 } \\
~ &  Conv2d & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256,kernel=3x3,stride=1,padding=1) } \\

\hline
\multirow{5}*{upsample\_block\_3} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256 } \\
~ &  Upsample(nearest\_interpolate) & \multicolumn{5}{|c|}{scale\_factor=2.0 } \\
~ &  Conv2d & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256,kernel=3x3,stride=1,padding=1) } \\

\hline
\multirow{5}*{upsample\_block\_4} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 128 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128 } \\
~ &  Upsample(nearest\_interpolate) & \multicolumn{5}{|c|}{scale\_factor=2.0 } \\
~ &  Conv2d & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128,kernel=3x3,stride=1,padding=1) } \\

\hline
\multirow{4}*{upsample\_block\_5} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128 } \\
~ &  ConvTranspose2d & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128, kennel:3x3,stride = 2} \\
 

\hline

\multirow{2}*{end} &  Normalize & \multicolumn{5}{|c|}{GroupNorm,num\_groups=32, num\_channels=512} \\
~ &  Conv2d & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 6, kernel: 3x3, stride: 1, pad: 1 } \\
\hline

\end{tabular}
\label{tab:decoder}
\end{table*}



\paragraph{Discriminator}
Following VQGAN, we define a 3-layer PatchGAN discriminator as in Pix2Pix \cite{pix2pix}. The discrimination takes the reconstructed output or the ground truth BEV map as input and outputs a prediction map to discriminate the reconstructed map from ground truth. It includes one input convolution layer using leaky ReLU as activation. It then includes three convolution layers with batch norm as normalization and leaky ReLU as activation. It finally contains an output convolution layer to output a one-channel prediction map.
 
\subsection{Latent Space Transformer}
The latent space transformer consists of a GPT transformer and a BEV feature extractor. The GPT transformer contains token embedding, feature embedding, and positional embedding. The token embedding is a learnable feature vector for each code in the codebook, and the positional embedding is a learnable feature vector for every position. The feature embedding is the output of the BEV feature extractor. The final embedding is the token embedding concatenated with feature embedding and then encoded with a positional embedding. The final embedding is then fed into 24 attention blocks, and each consists of one vanilla multi-head masked self-attention layer with 16 heads, three mlp layers, and layer norm. As in GPT, a causal mask ensures that attention is only applied to the past in the input sequence.

We present the detailed parameter of GPT in Tab.~\ref{tab:transformer}. The BEV feature extractor shares a similar architecture as the encoder. We present the detailed architecture in Tab. ~\ref{tab:feature}. 


\begin{table}[h] \centering
\caption{Architecture for Transformer}
\begin{tabular}{|c|c|}
\hline
parameters & value \\
\hline
vocab\_size & 1024 \\
\hline
block\_size(context\_size) & 512 \\
\hline
n\_layer & 24 \\
\hline
n\_head & 16 \\
\hline
n\_embd & 1024\\
\hline
\end{tabular}
\label{tab:transformer}

\end{table}



\begin{table*}[!t]
\caption{Architecture for BEV Feature Extarctor}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{layers} & \multicolumn{5}{|c|}{parameters} \\
\hline
input & Conv2d & \multicolumn{5}{|c|}{in\_ch:80/256, out\_ch: 128, kernel: 3x3, stride: 1, pad: 1 } \\
\hline

\multirow{3}*{downsample\_block\_1} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128 } \\
~ &  Downsample(Conv2d) & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128,kernel:3x3, stride:2, padding=((0,1,0,1),val=0) } \\
\hline
\multirow{3}*{downsample\_block\_2} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128 } \\
~ &  Downsample(Conv2d) & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 128,kernel:3x3, stride:2, padding=((0,1,0,1),val=0) } \\
\hline
\multirow{3}*{downsample\_block\_3} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:128, out\_ch: 256 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256 } \\
~ &  Downsample(Conv2d) & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256,kernel:3x3, stride:2, padding=((0,1,0,1),val=0) } \\
\hline
\multirow{2}*{downsample\_block\_4} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 512 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:256, out\_ch: 256 } \\
\hline
\multirow{3}*{middle} &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:512, out\_ch: 512 } \\
~ &  AttnBlock & \multicolumn{5}{|c|}{in\_ch:512 } \\
~ &  ResnetBlock & \multicolumn{5}{|c|}{in\_ch:512, out\_ch: 512 } \\
\hline
\multirow{3}*{end} &  Normalize & \multicolumn{5}{|c|}{GroupNorm,num\_groups=32, num\_channels=512} \\

~ &  Activation & \multicolumn{5}{|c|}{x*sigmoid(x)} \\

~ &  Conv2d & \multicolumn{5}{|c|}{in\_ch:512, out\_ch: 256, kernel: 3x3, stride: 1, pad: 1} \\
\hline


\end{tabular}
\label{tab:feature}
\end{table*}




==> supp_sec/qual.tex <==
\section{Additional Qualitative Results}
\label{sec:qual}
\subsection{Map Segmentation as Generation}

We provide additional Qualitative results for BEV map segmentation in Fig.~\ref{Additional_qual_L1} \ref{Additional_qual_L2} \ref{Additional_qual_C1} \ref{Additional_qual_C2}. The figures show that our model consistently generates results with better accuracy and realism than the baseline.  For instance, the fourth row of Fig.~\ref{Additional_qual_L1} demonstrates our approach preserves a realistic layout of a complicated multi-way intersection, with straight and complete lane boundaries, well-structured cross-walks as well as complete sidewalks, while the baseline's estimate is significantly noisier. In addition, the first row of Fig.~\ref{Additional_qual_L2} demonstrates our approach can complete the vertical layout of the road at the intersection despite limited sensor input. The generated vertical layout also preserves a realistic layout with well-structured lanes, crosswalks, and sidewalks. For another example, the first row in Fig.~\ref{Additional_qual_C2} demonstrates our approach generates correct and regular spacing of the lane boundaries, as well as smoother boundaries of sidewalks and roads than the camera baseline. 


In addition, we provide more diversity and uncertainty calibration results in Fig.~\ref{Additional Sampling Diversity} and ~\ref{Additional_Uncertainty Calibration}. Fig.~\ref{Additional Sampling Diversity} demonstrates that MapPrior can generate multiple diverse results, which can be aggregated into an accurate uncertainty map. Fig.~\ref{Additional_Uncertainty Calibration} shows that MapPrior's uncertainty map aligns better with the error map in different scenes.

 \begin{figure*}[!t] \centering 
 \begin{tabular}{ccccc} \centering
 \includegraphics[width=0.19\textwidth]{fig/random_samples/lidar_order_262.png}
 &\includegraphics[width=0.19\textwidth]{fig/random_samples/nos_262.png}
 &\includegraphics[width=0.19\textwidth]{fig/random_samples/res_262.png}
&\includegraphics[width=0.19\textwidth]{fig/random_samples/gt_262.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/random_samples/lidar_order_332.png}
 &\includegraphics[width=0.19\textwidth]{fig/random_samples/nos_332.png}
 &\includegraphics[width=0.19\textwidth]{fig/random_samples/res_332.png}
&\includegraphics[width=0.19\textwidth]{fig/random_samples/gt_332.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/random_samples/lidar_order_1500.png}
 &\includegraphics[width=0.19\textwidth]{fig/random_samples/nos_1500.png}
 &\includegraphics[width=0.19\textwidth]{fig/random_samples/res_1500.png}
&\includegraphics[width=0.19\textwidth]{fig/random_samples/gt_1500.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/random_samples/lidar_order_1520.png}
 &\includegraphics[width=0.19\textwidth]{fig/random_samples/nos_1520.png}
 &\includegraphics[width=0.19\textwidth]{fig/random_samples/res_1520.png}
&\includegraphics[width=0.19\textwidth]{fig/random_samples/gt_1520.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/random_samples/lidar_order_1600.png}
 &\includegraphics[width=0.19\textwidth]{fig/random_samples/nos_1600.png}
 &\includegraphics[width=0.19\textwidth]{fig/random_samples/res_1600.png}
&\includegraphics[width=0.19\textwidth]{fig/random_samples/gt_1600.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/L/lidar_order_2002.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/L/nos_2002.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/L/res_2002.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2002.png}
\\

Input & BEVFusion-L & MapPrior-L (Ours) & GT
 \end{tabular}
 \caption{Additional results of BEV map segmentation on
nuScenes}

 \label{Additional_qual_L1}
 \vspace{-4pt}
 \end{figure*}

 \begin{figure*}[!t] \centering 
 \begin{tabular}{ccccc} \centering

 \includegraphics[width=0.19\textwidth]{fig/more_samples/L/lidar_order_2142.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/L/nos_2142.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/L/res_2142.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2142.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/L/lidar_order_2042.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/L/nos_2042.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/L/res_2042.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2042.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/L/lidar_order_2362.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/L/nos_2362.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/L/res_2362.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2362.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/L/lidar_order_2202.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/L/nos_2202.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/L/res_2202.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2202.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/L/lidar_order_2302.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/L/nos_2302.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/L/res_2302.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2302.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/L/lidar_order_2402.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/L/nos_2402.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/L/res_2402.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2402.png}
\\
Input & BEVFusion-L & MapPrior-L (Ours) & GT
 \end{tabular}
 \caption{Additional Lidar results of BEV map segmentation on
nuScenes, continued}
 \label{Additional_qual_L2}
 \vspace{-4pt}
 \end{figure*}

 \begin{figure*}[!t] \centering 
 \begin{tabular}{ccccc} \centering
 \includegraphics[width=0.19\textwidth]{fig/more_samples/C/camera_order_2002.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/nos_2002.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/res_2002.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2002.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/C/camera_order_2022.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/nos_2022.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/res_2022.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2022.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/C/camera_order_2302.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/nos_2302.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/res_2302.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2302.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/C/camera_order_2602.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/nos_2602.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/res_2602.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2602.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/C/camera_order_2502.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/nos_2502.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/res_2502.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2502.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/C/camera_order_2562.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/nos_2562.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/res_2562.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2562.png}
\\
Input & BEVFusion-C & MapPrior-L (Ours) & GT
 \end{tabular}
 \caption{Additional Camera results of BEV map segmentation on
nuScenes}

 \label{Additional_qual_C1}
 \vspace{-4pt}
 \end{figure*}


 \begin{figure*}[!t] \centering 
 \begin{tabular}{ccccc} \centering
 \includegraphics[width=0.19\textwidth]{fig/more_samples/C/camera_order_2142.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/nos_2142.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/res_2142.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2142.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/C/camera_order_2042.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/nos_2042.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/res_2042.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2042.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/C/camera_order_2362.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/nos_2362.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/res_2362.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2362.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/C/camera_order_2202.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/nos_2202.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/res_2202.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2202.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/C/camera_order_2302.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/nos_2302.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/res_2302.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2302.png}
\\
 \includegraphics[width=0.19\textwidth]{fig/more_samples/C/camera_order_2402.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/nos_2402.png}
 &\includegraphics[width=0.19\textwidth]{fig/more_samples/C/res_2402.png}
&\includegraphics[width=0.19\textwidth]{fig/more_samples/GT/gt_2402.png}
\\
Input & BEVFusion-C & MapPrior-C (Ours) & GT
 \end{tabular}
 \caption{Additional Camera results of BEV map segmentation on
nuScenes, continued}

 \label{Additional_qual_C2}
 \vspace{-4pt}
 \end{figure*}




 

 \begin{figure*}[b] \centering 
 \begin{tabular}{cccccc} \centering
 \includegraphics[width=0.15\textwidth]{fig/diverse_res/lidar_42.png}
 &\includegraphics[width=0.15\textwidth]{fig/diverse_res/gt_42.png}
 &\includegraphics[width=0.15\textwidth]{fig/diverse_res_C/res_42_step_1.png}
&\includegraphics[width=0.15\textwidth]{fig/diverse_res/res_42_step_9.png}
&\includegraphics[width=0.15\textwidth]{fig/diverse_res/res_42_step_5.png}
&\includegraphics[width=0.15\textwidth]{fig/diverse_res/res_uncertainty42.png} 
\\
 \includegraphics[width=0.15\textwidth]{fig/diverse_res/lidar_22.png}
 &\includegraphics[width=0.15\textwidth]{fig/diverse_res/gt_22.png}
 &\includegraphics[width=0.15\textwidth]{fig/diverse_res_C/res_22_step_1.png}
&\includegraphics[width=0.15\textwidth]{fig/diverse_res/res_22_step_9.png}
&\includegraphics[width=0.15\textwidth]{fig/diverse_res/res_22_step_5.png}
&\includegraphics[width=0.15\textwidth]{fig/diverse_res/res_uncertainty22.png} 
\\

\includegraphics[width=0.15\textwidth]{fig/diverse_res/lidar_102.png}
 &\includegraphics[width=0.15\textwidth]{fig/diverse_res/gt_102.png}
 &\includegraphics[width=0.15\textwidth]{fig/diverse_res_C/res_102_step_9.png}
&\includegraphics[width=0.15\textwidth]{fig/diverse_res/res_102_step_1.png}
&\includegraphics[width=0.15\textwidth]{fig/diverse_res/res_102_step_5.png}
&\includegraphics[width=0.15\textwidth]{fig/diverse_res/res_uncertainty102.png}
\\
Input & GT & Our Sample 1 & Our Sample 2 & Our Sample 3 &  Uncertainty Map
 \end{tabular}
 \caption{Additional Qualitative results of diversity on NuScenes.}

 \label{Additional Sampling Diversity}
 \vspace{-4pt}
 \end{figure*}




 \begin{figure*}[b] \centering 
 \begin{tabular}{ccccccc} \centering


\includegraphics[width=0.12\textwidth]{fig/diverse_res/lidar_42.png} &
 \includegraphics[width=0.12\textwidth]{fig/diverse_res/nos_42.png} &  
 \includegraphics[width=0.12\textwidth]{fig/diverse_res/nos_uncertainty42.png} & 
 \includegraphics[width=0.12\textwidth]{fig/diverse_res/nos_errormap42.png} & 
 \includegraphics[width=0.12\textwidth]{fig/diverse_res_C/res_42_step_9.png} &  
 \includegraphics[width=0.12\textwidth]{fig/diverse_res/res_uncertainty42.png} &
  \includegraphics[width=0.12\textwidth]{fig/diverse_res/res_errormap42.png} \\
  
\includegraphics[width=0.12\textwidth]{fig/diverse_res/lidar_82.png} & 
 \includegraphics[width=0.12\textwidth]{fig/diverse_res/nos_82.png} &  
 \includegraphics[width=0.12\textwidth]{fig/diverse_res/nos_uncertainty82.png} & 
 \includegraphics[width=0.12\textwidth]{fig/diverse_res/nos_errormap82.png} & 
 \includegraphics[width=0.12\textwidth]{fig/diverse_res_C/res_82_step_9.png} &  
 \includegraphics[width=0.12\textwidth]{fig/diverse_res/res_uncertainty82.png} &
  \includegraphics[width=0.12\textwidth]{fig/diverse_res/res_errormap82.png} \\
 
\includegraphics[width=0.12\textwidth]{fig/random_samples/lidar_0.png} & 
 \includegraphics[width=0.12\textwidth]{fig/diverse_res/nos_2.png} &  
 \includegraphics[width=0.12\textwidth]{fig/diverse_res/nos_uncertainty2.png} & 
 \includegraphics[width=0.12\textwidth]{fig/diverse_res/nos_errormap2.png} & 
 \includegraphics[width=0.12\textwidth]{fig/diverse_res_C/res_2_step_9.png} &  
 \includegraphics[width=0.12\textwidth]{fig/diverse_res/res_uncertainty2.png} &
  \includegraphics[width=0.12\textwidth]{fig/diverse_res/res_errormap2.png} \\
  
 \multirow{2.5}{*}{LiDAR} &
 Prediction & Uncertainty & Error Map & Prediction & Uncertainty & Error Map 
 
 \\
 \cmidrule(lr){2-4}
 \cmidrule(lr){5-7}
 
 & \multicolumn{3}{c}{BEVFusion-L}
 & \multicolumn{3}{c}{MapPrior}
 \\

 \end{tabular}
 \caption{Additional results on uncertainty and error map comparison}
 \label{Additional_Uncertainty Calibration}
 \vspace{-8pt}
 \end{figure*}


\subsection{Failure Cases}
\label{sec:Failure}
Despite the overall improved IoU score in the benchmark, MapPrior can have a lower IoU score than the baseline model in certain cases. 
For example, in Fig.~\ref{fail}, there is a complicated layout distant from the ego car. In such cases, predictive models tend to make empty predictions.
In contrast, MapPrior makes a realistic generation of possible traffic layouts. However, this may lead to significant false positives and a lower IoU score than an empty layout prediction. The better-calibrated confidence score that MapPrior provides should help the downstream planner module be aware of the uncertain areas in this situation. 

 \begin{figure*}[h] \centering 
 \begin{tabular}{ccc} 


 \includegraphics[width=0.13\textwidth]{fig/random_samples/nos_200.png}
 &\includegraphics[width=0.13\textwidth]{fig/random_samples/res_200.png}
&\includegraphics[width=0.13\textwidth]{fig/random_samples/gt_200.png}
\\

 \includegraphics[width=0.13\textwidth]{fig/random_samples/nos_242.png}
 &\includegraphics[width=0.13\textwidth]{fig/random_samples/res_242.png}
&\includegraphics[width=0.13\textwidth]{fig/random_samples/gt_242.png}
\\


BEVFusion-L & MapPrior-L (Ours) & GT
 \end{tabular}
 \caption{Failure Cases}

 \label{fail}

 \end{figure*}



==> supp_sec/quant.tex <==
\section{Additional Quantitative Results}
\label{sec:quant}

\subsection{Expected calibration error clarification}
We would like to mention that the main paper calculates the expected calibration error (ECE) by evaluating the average rooted mean-squared error between the samples' accuracy and confidence for each bin. This calculation follows the method proposed in "Verified Uncertainty Calibration" \cite{newer_ECE} (Eq. 1). 
Strictly speaking, we should cite Kumar et al.~\cite{newer_ECE} instead of Guo et al.~\cite{ECE_Score} for the ECE calculation. This is because Guo et al. use the mean absolute error instead of the mean squared error, and their ECE score is given by:
$ \texttt{ECE}(B) = \sum_{b=1}^{B} \frac{n_b | \texttt{acc}(b) - \texttt{conf}(b) |_1}{n}.$
We will correct this mis-citation in the next revision of the paper. In addition, to provide a comprehensive understanding, we also compute the original ECE score following Guo et al. \cite{ECE_Score}. Under this metric, our method, MapPrior-L still significantly outperforms the strongest baseline, with scores of 0.021 for MapPrior-L and 0.066 for BEVFusion-L.








